Training With Data Dependent Dynamic Learning Rates

Recently many first and second order variants of SGD have been proposed to facilitate training of Deep Neural Networks (DNNs). A common limitation of these works stem from the fact that they use the same learning rate across all instances present in the dataset. This setting is widely adopted under the assumption that loss functions for each instance are similar in nature, and hence, a common learning rate can be used. In this work, we relax this assumption and propose an optimization framework which accounts for difference in loss function characteristics across instances. More specifically, our optimizer learns a dynamic learning rate for each instance present in the dataset. Learning a dynamic learning rate for each instance allows our optimization framework to focus on different modes of training data during optimization. When applied to an image classification task, across different CNN architectures, learning dynamic learning rates leads to consistent gains over standard optimizers. When applied to a dataset containing corrupt instances, our framework reduces the learning rates on noisy instances, and improves over the state-of-the-art. Finally, we show that our optimization framework can be used for personalization of a machine learning model towards a known targeted data distribution.

==> tex_files/method_neurips.tex <==
\section{Learning a Dynamic Curriculum via Data Parameters}
%\begin{figure}
%\centering
%\includegraphics[width=0.5\linewidth]{./figures/model_overview.png}
%\caption{Eric Clapton}
%\end{figure}
As suggested earlier, the main intuition behind our idea is simple: each class and data point in the 
training set has a parameter associated to it, which weighs the contribution of that class or data point in the gradient update of model parameters. 
In contrast to existing works which set these parameters with a heuristic, in our work these parameters are learnable and are learnt along with the model parameters.
Unlike model parameters which are involved during training and inference, data parameters are only involved during training. 
Therefore, using data parameters during training does not affect the model complexity and run-time at inference.
In the next section we formalize this intuition for class-level curriculum, followed by instance-level curriculum.

\subsection{Learning curriculum over classes}
\label{sec:class_curriculum}
We first describe learning a dynamic curriculum over classes where the contribution of each sample to the model learning is determined by its class. 
This curriculum favors learning from easier classes at the earlier stages of training. The curriculum over classes is dynamic and is controlled by the
class-level data parameters, which are also updated via the training process. In what follows, we will refer to class-level data parameters as class-parameters.

Let $\left\{\left(\mathbf{x}^i, y^i\right)\right\}^N_{i=1}$ denote the data, where $\mathbf{x}^i \in \mathbb{R}^d$ denotes 
a single data point and $y^i \in \{1, ..., k\}$ denotes its target label.
Let $\sigma^{class} \in \mathbb{R}^k$ denote the class parameters for the classes in the dataset.
We denote the neural network function mapping the input data $\mathbf{x}^i$ to 
logits $\mathbf{z}^i \in \mathbb{R}^{k}$ as $z^i = f_{\theta}(\mathbf{x}^i)$ where $\theta$ are the model parameters.
During training, we pass the input sample  $\mathbf{x}^i$ through the DNN, and
compute its corresponding logits $\mathbf{z}^i$, but instead of computing the softmax directly on the logits, 
we scale the logits of the instance with parameter corresponding to the target class, $\sigma^{class}_{y^i}$.
Note, scaling of logits with the parameter of target class can be interpreted as a temperature scaling of logits.
The cross-entropy loss for a data point $\mathbf{x}^i$ can then be written as
\begin{equation}
\begin{split}
L^i &= -\log(p^i_{{y^i}}) \\
p^i_{{y^i}} &= \frac{\exp(z^i_{{y^i}}/ \sigma_{{y^i}}^{class})} {\sum_{j} \exp(z^i_j/\sigma_{{y^i}}^{class})}
\end{split}
\label{eq:new_probs}
\end{equation}
where $p^i_{{y^i}}, z^i_{{y^i}}$ and $\sigma_{{y^i}}^{class}$ denote probability, logit and parameter of the target class ${y^i}$ for data point $\mathbf{x}_i$
respectively. If we set all class parameters to one, i.e.\ $\sigma^{class}_j = 1, j=1 \ldots k$, we recover the gradient for the standard cross-entropy loss. 

During training we solve
\begin{equation}
\min_{\theta, \sigma^{class}} \frac{1}{N} \sum_{i=1}^N L^i
\label{eq:optimization}
\end{equation}
where in addition to the model parameters, $\theta$, we also optimize the class-level parametres, $\sigma^{class}$. 

The gradient of the loss with respect to logits is given by:
\begin{equation}
\frac{\partial L^i}{\partial z^i_j} = \frac{p^i_j - 1(j = {y^i})}{\sigma_{{y^i}}^{class}}
\label{eq:partial_logits}
\end{equation}
where $1(j = {y^i})$ means value $1$ when $j = {y^i}$ and value $0$ otherwise. The gradient of the loss with respect to the parameter of target class is given by:
\begin{equation}
\begin{split}
\frac{\partial L^i}{\partial \sigma^{class}_{{y^i}}} &= \frac{(1 - p^i_{{y^i}})}{(\sigma^{class}_{{y^i}})^2} \Big(z^i_{{y^i}} - \sum_{j \neq
{y^i}} q^i_j z^i_j\Big)
\end{split}
\label{eq:gradient_sigma_pd_over_k}
\end{equation}
 where $q^i_j = \frac{p^i_j}{1-p^i_{{y^i}}}$ is the probability distribution over non-target classes (indexed by $j$, with $j \neq {y^i}$).
% A more detailed derivation for the update rule is provided in the supplementary material.


\paragraph{Effect of class parameters on learning: } 

The class parameters are updated with the negative of the gradient given in equation (\ref{eq:gradient_sigma_pd_over_k}), where the parameter
corresponding to target class $\sigma^{class}_{{y^i}}$ will increase if the logit of 
the target class is less than the expected value of logits on non-target classes (i.\,e. $ z^i_{{y^i}} <
\sum_{j \neq {y^i}} q^i_j z^i_j$) and vice-versa. 
Therefore, during the course of learning, if data-points of a certain class are being misclassified,
the gradient update on class parameters gradually increases the parameter associated with this class. 
Increasing the class parameter, flattens the curvature of the loss function for instances of that class, 
thereby decaying the gradients w.r.t. logits (see equation (\ref{eq:partial_logits})).
Decreasing the class parameter has an inverse effect, and accelerates the learning. 
 
\subsection{Learning curriculum over instances}
In the previous section, we have detailed how we can learn a dynamic curriculum over classes of a dataset. 
A natural extension of this framework is to have a dynamic curriculum over the instances in the dataset. 
In this case, in equation (\ref{eq:new_probs}), rather than having class parameters for each class $\sigma^{class}_j, j \in \{1, \ldots , k\}$, 
we can have a instance parameters for each sample present in the dataset, $\sigma^{inst}_i, i \in \{1, \ldots , N\}$. 

This parameterization helps us to learn a curriculum over instances of a class, which is useful when instances within a class have different levels of difficulty. 
For instance, consider the task of classifying images of an object. 
In some instances, the object could be fully visible (easy), while in others, it could be occluded by other objects (hard). 
Another task is learning with noisy/corrupt labels. In this setting, labels of some instances would be consistent with the input (easy), while labels
of some instances would not be consistent (hard). 
%In our experiments we show that, learning a dynamic curriculum over instances, learns from the easier samples first; 
%In the presence of noisy labels where some instances of the training data would be consistent with their target labels, 
%while some instances would not be consistent. 
In our experiments, we show that the learning of a curriculum over instances learns to ignore the noisy samples.

We can also learn a joint curriculum over classes and instances to have the benefits of both. In this case, during training, the parameter for a data point
$\mathbf{x}^i$ is set as the sum of its target's class paramter $\sigma_{y^i}$ and its own instance parameter $\sigma^{inst}_i$ 
i.e.\ $\sigma_i^{*} = \sigma_{{y^i}}^{class} + \sigma^{inst}_i$.
In this setting, the gradient of the loss with respect to the logits (as in equation
\ref{eq:partial_logits}) can be expressed as $\frac{\partial L^i}{\partial z^i_j} = \frac{p^i_j - 1(j = {y^i})}{\sigma_i^{*}}$.
Since the effective parameter of an instance is formed by the addition of class and instance level parameters, 
the gradient  for these parameters for a data point $\mathbf{x}^i$ is the same and is denoted by:% $\frac{\partial L_i}{\partial \sigma_i^{*}}$:
\begin{equation}
\begin{split}
\frac{\partial L^i}{\partial \sigma_i^{*}} &= \frac{(1 - p^i_{{y^i}})}{(\sigma_i^*)^2} \Big(z^i_{{y^i}} - \sum_{j \neq {y^i}} q^i_j z^i_j\Big) \\
%\frac{\partial L}{\partial \sigma^{c}} &= \frac{1}{n_c}\sum^{n_c}_{\substack{i\\ {y^i}_i = c}} \frac{\partial L_i}{\partial \sigma_i^*} \\
%\frac{\partial L}{\partial \sigma^{inst}_i} &= \frac{\partial L_i}{\partial \sigma_i^*} 
\end{split}
\end{equation}
However note, during training, instance parameters collect their gradient from individual samples (when sampled in a mini-batch), 
while class parameters average the gradient from all samples of the class present in a mini-batch.


\paragraph{Inference with data parameters:} 
As explained earlier, during training, we modify the logits of a sample with data parameters (class or instance parameters).
During inference, we do not have parameters on the test set, and hence do not scale the logits with a data parameter.
Not scaling the logits, has no affect on the argmax of softmax, but the classification probability is uncalibrated.
If one is interested in calibrated output, calibration can be done on a held-out validation set \cite{guo2017calibration}.
Note this modus operandi, of not scaling logits at inference, maintains our claim: use of data parameters does not affect the model's capacity and run-time at infernece. 



%where $\frac{\partial L_i}{\partial \sigma_i^{*}} = \frac{(1 - p_i^{{y^i}})}{(\sigma_i^*)^2} \Big(z_i^{{y^i}} - \sum_{j \neq {y^i}} q_i^j 
%z_i^j\Big)$ (see equation \ref{eq:gradient_sigma_pd_over_k}).
%where $\frac{\partial L}{\partial \sigma^{c}}$ and $n_c$ denote the gradient for temperature parameter of class $c$, and number of data points of class $c$ in a 
%mini-batch respectively.
%\subsection{Comparison with learning an explicit weighting per data-point}
%\subsection{Comparison with label-smoothing}
%\subsection{Memorization vs Generalization}
%
%\subsection{Comparison to Uncertainty modelling}
%\subsection{Comparison with ADAM}
%\newpage
%\subsection{Modifying the loss function}
%\begin{wrapfigure}{r}{5cm}
%\vspace{-0.5in}
%%\begin{figure}
%    \centering
%   \includegraphics[width=\linewidth]{./figures/loss_vs_diff_sigmas.png}
%   %\caption{Variation in cross-entropy loss as a function of temperature parameter $\sigma$. 
%   %When network predictions are worse than random, temperature parameters 
%   %attain a higher value to reduce the loss and dampen the gradients. See text for details.}
%%\end{figure}
%\vspace{-0.2in}
%\end{wrapfigure} 
%In this section we illustrate the connection between temperature of a softmax and its affect on the resulting loss function.
%In \cite{gao2017properties}, authors have shown that softmax function is $L$-Lipschitz with $L = 1/T$, where $T$ is the temperature used in the softmax.
% We illustrate this with a toy example which has three classes.   
% In the figure on the right, using the blue curve,  we plot the cross-entropy loss of a target class on the y-axis, 
% while varying the probability of target class with temperature set to 1 on the x-axis.  
% Now, keeping the inputt logits to softmax fixed, we vary the temperature, and trace the resulting loss functions (color-coded by temperature).
%As seen from figure, using a high temperature (black curve) results in a flatter loss function, whereas using a low temperature (green curve) results in a
%steeper loss function. Therefore, in our framework, optimizing class and instance temperature parameters along with model parameters, 
%modifies the loss function for each class and instance based on the current state of model, yielding a dynamic curriculum.  
%In our experimental section, we validate this hypothesis, and show the dynamic curriculum over different classes and instances during the course of optimization. 
%


